The FAST Ultra-Deep Survey (FUDS): observational strategy, calibration and data reduction

The FAST Ultra-Deep Survey (FUDS) is a blind survey that aims for the direct detection of HI in galaxies at redshifts $z<0.42$. The survey uses the multibeam receiver on the Five Hundred Meter Aperture Spherical Telescope (FAST) to map six regions, each of size 0.72 deg$^2$ at high sensitivity ($\sim 50 \mu$Jy) and high frequency resolution (23 kHz). The survey will enable studies of the evolution of galaxies and their HI content with an eventual sample size of $\sim 1000$. We present the science goals, observing strategy, the effects of radio frequency interference (RFI) at the FAST site, our mitigation strategies and the methods for calibration, data reduction and imaging as applied to initial data. The observations and reductions for the first field, FUDS0, are completed, with around 128 HI galaxies detected in a preliminary analysis. Example spectra are given in this paper, including a comparison with data from the overlapping GAL2577 field of Arecibo Ultra-Deep Survey (AUDS).

==> References.tex <==
@ARTICLE{2016JAI.....541001H,
       author = {{Hickish}, Jack and {Abdurashidova}, Zuhra and {Ali}, Zaki and {Buch}, Kaushal D. and {Chaudhari}, Sandeep C. and {Chen}, Hong and {Dexter}, Matthew and {Domagalski}, Rachel Simone and {Ford}, John and {Foster}, Griffin and {George}, David and {Greenberg}, Joe and {Greenhill}, Lincoln and {Isaacson}, Adam and {Jiang}, Homin and {Jones}, Glenn and {Kapp}, Francois and {Kriel}, Henno and {Lacasse}, Rich and {Lutomirski}, Andrew and {MacMahon}, David and {Manley}, Jason and {Martens}, Andrew and {McCullough}, Randy and {Muley}, Mekhala V. and {New}, Wesley and {Parsons}, Aaron and {Price}, Daniel C. and {Primiani}, Rurik A. and {Ray}, Jason and {Siemion}, Andrew and {van Tonder}, Verees{\'e} and {Vertatschitsch}, Laura and {Wagner}, Mark and {Weintroub}, Jonathan and {Werthimer}, Dan},
        title = "{A Decade of Developing Radio-Astronomy Instrumentation using CASPER Open-Source Technology}",
      journal = {Journal of Astronomical Instrumentation},
     keywords = {CASPER, digital signal processing, radio-astronomy, instrumentation, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = dec,
       volume = {5},
       number = {4},
          eid = {1641001-12},
        pages = {1641001-12},
          doi = {10.1142/S2251171716410014},
archivePrefix = {arXiv},
       eprint = {1611.01826},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JAI.....541001H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014PASA...31....7C,
       author = {{Calabretta}, Mark R. and {Staveley-Smith}, Lister and {Barnes}, David G.},
        title = "{A New 1.4 GHz Radio Continuum Map of the Sky South of Declination +25{\textdegree}}",
      journal = {\pasa},
     keywords = {atlases, cosmic background radiation, methods: data analysis, radio continuum: general, surveys, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jan,
       volume = {31},
          eid = {e007},
        pages = {e007},
          doi = {10.1017/pasa.2013.36},
archivePrefix = {arXiv},
       eprint = {1310.2414},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PASA...31....7C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1965ITAP...13..660R,
       author = {{Ruze}, Johit},
        title = "{Lateral-feed displacement in a paraboloid}",
      journal = {IEEE Transactions on Antennas and Propagation},
         year = 1965,
        month = sep,
       volume = {13},
       number = {5},
        pages = {660-665},
          doi = {10.1109/TAP.1965.1138514},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1965ITAP...13..660R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016MNRAS.455.1574J,
       author = {{Jones}, Michael G. and {Haynes}, Martha P. and {Giovanelli}, Riccardo and {Papastergis}, Emmanouil},
        title = "{When is stacking confusing? The impact of confusion on stacking in deep H I galaxy surveys}",
      journal = {\mnras},
     keywords = {surveys, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jan,
       volume = {455},
       number = {2},
        pages = {1574-1583},
          doi = {10.1093/mnras/stv2394},
archivePrefix = {arXiv},
       eprint = {1510.03854},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.455.1574J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018A&A...619A..89B,
       author = {{Butcher}, Z. and {Schneider}, S. and {van Driel}, W. and {Lehnert}, M.~D.},
        title = "{Bivariate luminosity-HI mass distribution function of galaxies based on the NIBLES survey}",
      journal = {\aap},
     keywords = {galaxies: luminosity function, mass function, galaxies: distances and redshifts, galaxies: evolution, galaxies: general, galaxies: fundamental parameters, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = nov,
       volume = {619},
          eid = {A89},
        pages = {A89},
          doi = {10.1051/0004-6361/201832659},
archivePrefix = {arXiv},
       eprint = {1809.03155},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...619A..89B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.445.2125M,
       author = {{McNaught-Roberts}, Tamsyn and {Norberg}, Peder and {Baugh}, Carlton and {Lacey}, Cedric and {Loveday}, J. and {Peacock}, J. and {Baldry}, I. and {Bland-Hawthorn}, J. and {Brough}, S. and {Driver}, Simon P. and {Robotham}, A.~S.~G. and {V{\'a}zquez-Mata}, J.~A.},
        title = "{Galaxy And Mass Assembly (GAMA): the dependence of the galaxy luminosity function on environment, redshift and colour}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: luminosity function, mass function, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = dec,
       volume = {445},
       number = {2},
        pages = {2125-2145},
          doi = {10.1093/mnras/stu1886},
archivePrefix = {arXiv},
       eprint = {1409.4681},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.445.2125M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016OJAp....1E...3L,
       author = {{Lake}, Sean E. and {Wright}, Edward L.},
        title = "{K-Corrections AN Examination of Their Contribution to the Uncertainty of Luminosity Measurements}",
      journal = {The Open Journal of Astrophysics},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Data Analysis, Statistics and Probability},
         year = 2016,
        month = oct,
       volume = {1},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.21105/astro.1603.07299},
archivePrefix = {arXiv},
       eprint = {1603.07299},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016OJAp....1E...3L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.369...25J,
       author = {{Jones}, D. Heath and {Peterson}, Bruce A. and {Colless}, Matthew and {Saunders}, Will},
        title = "{Near-infrared and optical luminosity functions from the 6dF Galaxy Survey}",
      journal = {\mnras},
     keywords = {surveys: galaxies: distances and redshifts: galaxies: luminosity function, mass function: cosmology: observations: large-scale structure of Universe, surveys, galaxies: distances and redshifts, galaxies: luminosity function, mass function, cosmology: observations, large-scale structure of Universe, Astrophysics},
         year = 2006,
        month = jun,
       volume = {369},
       number = {1},
        pages = {25-42},
          doi = {10.1111/j.1365-2966.2006.10291.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603609},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.369...25J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...558A..33A,
       author = {{Astropy Collaboration} and {Robitaille}, Thomas P. and {Tollerud}, Erik J. and {Greenfield}, Perry and {Droettboom}, Michael and {Bray}, Erik and {Aldcroft}, Tom and {Davis}, Matt and {Ginsburg}, Adam and {Price-Whelan}, Adrian M. and {Kerzendorf}, Wolfgang E. and {Conley}, Alexander and {Crighton}, Neil and {Barbary}, Kyle and {Muna}, Demitri and {Ferguson}, Henry and {Grollier}, Fr{\'e}d{\'e}ric and {Parikh}, Madhura M. and {Nair}, Prasanth H. and {Unther}, Hans M. and {Deil}, Christoph and {Woillez}, Julien and {Conseil}, Simon and {Kramer}, Roban and {Turner}, James E.~H. and {Singer}, Leo and {Fox}, Ryan and {Weaver}, Benjamin A. and {Zabalza}, Victor and {Edwards}, Zachary I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and {Casey}, Andrew R. and {Crawford}, Steven M. and {Dencheva}, Nadia and {Ely}, Justin and {Jenness}, Tim and {Labrie}, Kathleen and {Lim}, Pey Lian and {Pierfederici}, Francesco and {Pontzen}, Andrew and {Ptak}, Andy and {Refsdal}, Brian and {Servillat}, Mathieu and {Streicher}, Ole},
        title = "{Astropy: A community Python package for astronomy}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2013,
        month = oct,
       volume = {558},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/201322068},
archivePrefix = {arXiv},
       eprint = {1307.6212},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..33A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018AJ....156..123A,
       author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H{o}}cz}, B.~M. and {G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and {Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and {Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and {P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and {Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and {Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and {Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and {Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and {Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and {Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'\i}guez}, J.~L. and {Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and {Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and {Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and {Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and {Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and {Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and {Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and {Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and {Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and {Ivezi{\'c}}, {\v{Z}}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and {Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and {Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and {Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and {Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and {Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and {Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and {Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and {Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and {Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and {Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and {Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and {Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and {Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and {Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and {Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and {van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and {Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and {Zabalza}, V. and {Astropy Contributors}},
        title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
      journal = {\aj},
     keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {156},
       number = {3},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-3881/aabc4f},
archivePrefix = {arXiv},
       eprint = {1801.02634},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2018AAS...23123107B,
       author = {{Baker}, Andrew J. and {Blyth}, Sarah and {Holwerda}, Benne W. and
         {LADUMA Team}},
        title = "{LADUMA: Looking At the Distant Universe with the MeerKAT Array}",
    booktitle = {American Astronomical Society Meeting Abstracts \#231},
         year = 2018,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {231},
        month = jan,
          eid = {231.07},
        pages = {231.07},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AAS...23123107B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.322..486B,
       author = {{Barnes}, D.~G. and {Staveley-Smith}, L. and {de Blok}, W.~J.~G. and
         {Oosterloo}, T. and {Stewart}, I.~M. and {Wright}, A.~E. and
         {Banks}, G.~D. and {Bhathal}, R. and {Boyce}, P.~J. and
         {Calabretta}, M.~R. and {Disney}, M.~J. and {Drinkwater}, M.~J. and
         {Ekers}, R.~D. and {Freeman}, K.~C. and {Gibson}, B.~K. and
         {Green}, A.~J. and {Haynes}, R.~F. and {te Lintel Hekkert}, P. and
         {Henning}, P.~A. and {Jerjen}, H. and {Juraszek}, S. and
         {Kesteven}, M.~J. and {Kilborn}, V.~A. and {Knezek}, P.~M. and
         {Koribalski}, B. and {Kraan-Korteweg}, R.~C. and {Malin}, D.~F. and
         {Marquarding}, M. and {Minchin}, R.~F. and {Mould}, J.~R. and
         {Price}, R.~M. and {Putman}, M.~E. and {Ryder}, S.~D. and
         {Sadler}, E.~M. and {Schr{\"o}der}, A. and {Stootman}, F. and
         {Webster}, R.~L. and {Wilson}, W.~E. and {Ye}, T.},
        title = "{The HI Parkes All Sky Survey: southern observations, calibration and robust imaging}",
      journal = {\mnras},
     keywords = {INSTRUMENTATION: DETECTORS, METHODS: OBSERVATIONAL, METHODS: STATISTICAL, TECHNIQUES: IMAGE PROCESSING, SURVEYS, RADIO LINES: GALAXIES},
         year = "2001",
        month = "Apr",
       volume = {322},
       number = {3},
        pages = {486-498},
          doi = {10.1046/j.1365-8711.2001.04102.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.322..486B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJS...75....1B,
       author = {{Becker}, Robert H. and {White}, Richard L. and {Edwards}, Alan L.},
        title = "{A New Catalog of 53,522 4.85 GHz Sources}",
      journal = {\apjs},
     keywords = {Astronomical Catalogs, Astronomical Spectroscopy, Extragalactic Radio Sources, Sky Surveys (Astronomy), Astronomical Photography, Data Processing, Image Processing, Northern Hemisphere, Reference Stars, Spectrum Analysis, Tables (Data), Astronomy, RADIO SOURCES: GENERAL},
         year = 1991,
        month = jan,
       volume = {75},
        pages = {1},
          doi = {10.1086/191529},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJS...75....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...882L...7B,
       author = {{Bera}, Apurba and {Kanekar}, Nissim and {Chengalur}, Jayaram N. and {Bagla}, Jasjeet S.},
        title = "{Atomic Hydrogen in Star-forming Galaxies at Intermediate Redshifts}",
      journal = {\apjl},
     keywords = {Galaxy evolution, Radio interferometry, Radio spectroscopy, Star formation, H I line emission, High-redshift galaxies, 594, 1346, 1359, 1569, 690, 734, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = sep,
       volume = {882},
       number = {1},
          eid = {L7},
        pages = {L7},
          doi = {10.3847/2041-8213/ab3656},
archivePrefix = {arXiv},
       eprint = {1909.05905},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...882L...7B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2016mks..confE...4B,
       author = {{Blyth}, S. and {Baker}, A.~J. and {Holwerda}, B. and {Bouchard}, A. and
         {Catinella}, B. and {Chemin}, L. and {Cunnama}, D. and {Dav{\'e}}, R. and
         {Faltenbacher}, A. and {February}, S. and {Fern{\'a}ndez}, X. and
         {Gawiser}, E. and {Heywood}, I. and {Kere{\v{s}}}, D. and
         {Kl{\"o}ckner}, H.~R. and {Lah}, P. and {Lochner}, M. and {Maddox}, N. and
         {Makhathini}, S. and {Moodley}, K. and {Morganti}, R. and
         {Obreschkow}, D. and {Oh}, S.~H. and {Pisano}, D.~J. and {Popping}, A. and
         {Popping}, G. and {Ravindranath}, S. and {Schinnerer}, E. and
         {Sheth}, K. and {Skelton}, R. and {Smith}, M. and {Srianand}, R. and
         {Staveley-Smith}, L. and {Vaccari}, M. and {Vaisanen}, P. and
         {Walter}, F. and {Rawlings}, S. and {Bassett}, B.~A. and
         {Bershady}, M.~A. and {Briggs}, F.~H. and {Crawford}, S.~M. and
         {Cress}, C.~M. and {Darling}, J.~K. and {Deane}, R.~P. and
         {de Blok}, G. and {Elson}, E.~C. and {Frank}, B.~S. and
         {Henning}, P.~A. and {Hess}, K.~M. and {Hughes}, J.~P. and
         {Jarvis}, M.~J. and {Kannappan}, S.~J. and {Katz}, N.~S. and
         {Kraan-Korteweg}, R.~C. and {Lehnert}, M.~D. and {Leroy}, A.~K. and
         {Meurer}, G.~R. and {Meyer}, M.~J. and {Pisano}, D.~J. and
         {Schr{\"o}der}, A.~C. and {Smirnov}, O.~M. and {Somerville}, R.~S. and
         {Stewart}, I.~M. and {van der Heyden}, K.~J. and {Verheijen}, M.~A.~W. and
         {Wilcots}, E.~M. and {Williams}, T.~B. and {Woudt}, P.~A. and
         {Wu}, J.~F. and {Zwaan}, M.~A. and {Zwart}, J.~T.~L. and
         {Oosterloo}, T.~A. and {van Drie}, W.},
        title = "{LADUMA: Looking at the Distant Universe with the MeerKAT Array}",
    booktitle = {MeerKAT Science: On the Pathway to the SKA},
         year = 2016,
        month = jan,
          eid = {4},
        pages = {4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016mks..confE...4B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.501.2608B,
       author = {{Busekool}, E. and {Verheijen}, M.~A.~W. and {van der Hulst}, J.~M. and {Tully}, R.~B. and {Trentham}, N. and {Zwaan}, M.~A.},
        title = "{The Ursa Major association of galaxies - VI: a relative dearth of gas-rich dwarf galaxies}",
      journal = {\mnras},
     keywords = {galaxies: clusters: individual: Ursa Major, galaxies: dwarf, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = feb,
       volume = {501},
       number = {2},
        pages = {2608-2626},
          doi = {10.1093/mnras/staa3582},
archivePrefix = {arXiv},
       eprint = {2012.03648},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.2608B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010Natur.466..463C,
       author = {{Chang}, Tzu-Ching and {Pen}, Ue-Li and {Bandura}, Kevin and
         {Peterson}, Jeffrey B.},
        title = "{An intensity map of hydrogen 21-cm emission at redshift z\raisebox{-0.5ex}\textasciitilde0.8}",
      journal = {\nat},
         year = 2010,
        month = jul,
       volume = {466},
       number = {7305},
        pages = {463-465},
          doi = {10.1038/nature09187},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.466..463C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...372..768C,
       author = {{Chengalur}, J.~N. and {Braun}, R. and {Wieringa}, M.},
        title = "{HI in Abell 3128}",
      journal = {\aap},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: CLUSTERS: INDIVIDUAL: A3128, GALAXIES: HI CONTENT, COSMOLOGY: OBSERVATIONS, RADIO LINES: GALAXIES, Astrophysics},
         year = 2001,
        month = jun,
       volume = {372},
        pages = {768-774},
          doi = {10.1051/0004-6361:20010547},
archivePrefix = {arXiv},
       eprint = {astro-ph/0104331},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...372..768C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007AJ....134.1245C,
       author = {{Cohen}, A.~S. and {Lane}, W.~M. and {Cotton}, W.~D. and {Kassim}, N.~E. and {Lazio}, T.~J.~W. and {Perley}, R.~A. and {Condon}, J.~J. and {Erickson}, W.~C.},
        title = "{The VLA Low-Frequency Sky Survey}",
      journal = {\aj},
     keywords = {atmospheric effects, catalogs, radio continuum: general, surveys, Astrophysics},
         year = 2007,
        month = sep,
       volume = {134},
       number = {3},
        pages = {1245-1262},
          doi = {10.1086/520719},
archivePrefix = {arXiv},
       eprint = {0706.1191},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AJ....134.1245C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998AJ....115.1693C,
       author = {{Condon}, J.~J. and {Cotton}, W.~D. and {Greisen}, E.~W. and {Yin}, Q.~F. and {Perley}, R.~A. and {Taylor}, G.~B. and {Broderick}, J.~J.},
        title = "{The NRAO VLA Sky Survey}",
      journal = {\aj},
     keywords = {CATALOGS, METHODS: DATA ANALYSIS, METHODS: OBSERVATIONAL, RADIO CONTINUUM, SURVEYS},
         year = 1998,
        month = may,
       volume = {115},
       number = {5},
        pages = {1693-1716},
          doi = {10.1086/300337},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998AJ....115.1693C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.446.3526C,
       author = {{Catinella}, Barbara and {Cortese}, Luca},
        title = "{HIGHz: a survey of the most H I-massive galaxies at z {\ensuremath{\sim}} 0.2}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: kinematics and dynamics, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {446},
       number = {4},
        pages = {3526-3544},
          doi = {10.1093/mnras/stu2241},
archivePrefix = {arXiv},
       eprint = {1410.7464},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.3526C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.476..875C,
       author = {{Catinella}, Barbara and {Saintonge}, Am{\'e}lie and
         {Janowiecki}, Steven and {Cortese}, Luca and {Dav{\'e}}, Romeel and
         {Lemonias}, Jenna J. and {Cooper}, Andrew P. and {Schiminovich}, David and
         {Hummels}, Cameron B. and {Fabello}, Silvia and {Ger{\'e}b}, Katinka and
         {Kilborn}, Virginia and {Wang}, Jing},
        title = "{xGASS: total cold gas scaling relations and molecular-to-atomic gas ratios of galaxies in the local Universe}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: ISM, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = may,
       volume = {476},
       number = {1},
        pages = {875-895},
          doi = {10.1093/mnras/sty089},
archivePrefix = {arXiv},
       eprint = {1802.02373},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476..875C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.467..115D,
       author = {{Dav{\'e}}, Romeel and {Rafieferantsoa}, Mika H. and
         {Thompson}, Robert J. and {Hopkins}, Philip F.},
        title = "{MUFASA: Galaxy star formation, gas, and metal properties across cosmic time}",
      journal = {\mnras},
     keywords = {galaxies: formation, galaxies: evolution, galaxies: star formation, galaxies: abundances, galaxies: ISM, methods: numerical, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = may,
       volume = {467},
       number = {1},
        pages = {115-132},
          doi = {10.1093/mnras/stx108},
archivePrefix = {arXiv},
       eprint = {1610.01626},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.467..115D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.433.1398D,
       author = {{Delhaize}, J. and {Meyer}, M.~J. and {Staveley-Smith}, L. and
         {Boyle}, B.~J.},
        title = "{Detection of H I in distant galaxies using spectral stacking}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, radio lines: galaxies, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {433},
       number = {2},
        pages = {1398-1410},
          doi = {10.1093/mnras/stt810},
archivePrefix = {arXiv},
       eprint = {1305.1968},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433.1398D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005AJ....129..220D,
       author = {{Donley}, J.~L. and {Staveley-Smith}, L. and {Kraan-Korteweg}, R.~C. and
         {Islas-Islas}, J.~M. and {Schr{\"o}der}, A. and {Henning}, P.~A. and
         {Koribalski}, B. and {Mader}, S. and {Stewart}, I.},
        title = "{The H I Parkes Zone of Avoidance Survey: The Northern Extension}",
      journal = {\aj},
     keywords = {Galaxies: Distances and Redshifts, Galaxies: Fundamental Parameters, Cosmology: Large-Scale Structure of Universe, Surveys, Astrophysics},
         year = 2005,
        month = jan,
       volume = {129},
       number = {1},
        pages = {220-238},
          doi = {10.1086/426320},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409570},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AJ....129..220D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996AJ....111.1945D,
       author = {{Douglas}, James N. and {Bash}, Frank N. and {Bozyan}, F. Arakel and {Torrence}, Geoffrey W. and {Wolfe}, Chip},
        title = "{The Texas Survey of Radio Sources Covering -35.5 degrees < declination < 71.5 degrees at 365 MHz}",
      journal = {\aj},
     keywords = {SURVEYS, RADIO LINES: GENERAL},
         year = 1996,
        month = may,
       volume = {111},
        pages = {1945},
          doi = {10.1086/117932},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996AJ....111.1945D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974AnAS...18..147F,
       author = {{Fanti}, C. and {Fanti}, R. and {Ficarra}, A. and {Padrielli}, L.},
        title = "{The B2 catalogue of radio sources - fourth part.}",
      journal = {\aaps},
         year = 1974,
        month = jan,
       volume = {18},
        pages = {147-156},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974A&AS...18..147F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...824L...1F,
       author = {{Fern{\'a}ndez}, Ximena and {Gim}, Hansung B. and {van Gorkom}, J.~H. and {Yun}, Min S. and {Momjian}, Emmanuel and {Popping}, Attila and {Chomiuk}, Laura and {Hess}, Kelley M. and {Hunt}, Lucas and {Kreckel}, Kathryn and {Lucero}, Danielle and {Maddox}, Natasha and {Oosterloo}, Tom and {Pisano}, D.~J. and {Verheijen}, M.~A.~W. and {Hales}, Christopher A. and {Chung}, Aeree and {Dodson}, Richard and {Golap}, Kumar and {Gross}, Julia and {Henning}, Patricia and {Hibbard}, John and {Jaff{\'e}}, Yara L. and {Donovan Meyer}, Jennifer and {Meyer}, Martin and {Sanchez-Barrantes}, Monica and {Schiminovich}, David and {Wicenec}, Andreas and {Wilcots}, Eric and {Bershady}, Matthew and {Scoville}, Nick and {Strader}, Jay and {Tremou}, Evangelia and {Salinas}, Ricardo and {Ch{\'a}vez}, Ricardo},
        title = "{Highest Redshift Image of Neutral Hydrogen in Emission: A CHILES Detection of a Starbursting Galaxy at z = 0.376}",
      journal = {\apjl},
     keywords = {galaxies: evolution, galaxies: starburst, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jun,
       volume = {824},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.3847/2041-8205/824/1/L1},
archivePrefix = {arXiv},
       eprint = {1606.00013},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824L...1F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...727...40F,
       author = {{Freudling}, Wolfram and {Staveley-Smith}, Lister and {Catinella}, Barbara and {Minchin}, Robert and {Calabretta}, Mark and {Momjian}, Emmanuel and {Zwaan}, Martin and {Meyer}, Martin and {O'Neil}, Karen},
        title = "{Deep 21 cm H I Observations at z {\ensuremath{\approx}} 0.1: The Precursor to the Arecibo Ultra Deep Survey}",
      journal = {\apj},
     keywords = {cosmology: observations, galaxies: evolution, radio lines: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = jan,
       volume = {727},
       number = {1},
          eid = {40},
        pages = {40},
          doi = {10.1088/0004-637X/727/1/40},
archivePrefix = {arXiv},
       eprint = {1011.0877},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...727...40F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJS...75.1011G,
       author = {{Gregory}, P.~C. and {Condon}, J.~J.},
        title = "{The 87GB Catalog of Radio Sources Covering 0 degrees < delta < +75 degrees at 4.85 GHz}",
      journal = {\apjs},
     keywords = {Astronomical Catalogs, Radio Sources (Astronomy), Evolution (Development), Radiant Flux Density, Radio Telescopes, Astronomy, RADIO SOURCES: GENERAL},
         year = 1991,
        month = apr,
       volume = {75},
        pages = {1011},
          doi = {10.1086/191559},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJS...75.1011G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005AJ....130.2598G,
       author = {{Giovanelli}, Riccardo and {Haynes}, Martha P. and {Kent}, Brian R. and {Perillat}, Philip and {Saintonge}, Amelie and {Brosch}, Noah and {Catinella}, Barbara and {Hoffman}, G. Lyle and {Stierwalt}, Sabrina and {Spekkens}, Kristine and {Lerner}, Mikael S. and {Masters}, Karen L. and {Momjian}, Emmanuel and {Rosenberg}, Jessica L. and {Springob}, Christopher M. and {Boselli}, Alessandro and {Charmandaris}, Vassilis and {Darling}, Jeremy K. and {Davies}, Jonathan and {Garcia Lambas}, Diego and {Gavazzi}, Giuseppe and {Giovanardi}, Carlo and {Hardy}, Eduardo and {Hunt}, Leslie K. and {Iovino}, Angela and {Karachentsev}, Igor D. and {Karachentseva}, Valentina E. and {Koopmann}, Rebecca A. and {Marinoni}, Christian and {Minchin}, Robert and {Muller}, Erik and {Putman}, Mary and {Pantoja}, Carmen and {Salzer}, John J. and {Scodeggio}, Marco and {Skillman}, Evan and {Solanes}, Jose M. and {Valotto}, Carlos and {van Driel}, Wim and {van Zee}, Liese},
        title = "{The Arecibo Legacy Fast ALFA Survey. I. Science Goals, Survey Design, and Strategy}",
      journal = {\aj},
     keywords = {Galaxies: Distances and Redshifts, Galaxies: Halos, Galaxies: Luminosity Function, Mass Function, Galaxies: Photometry, Galaxies: Spiral, Radio Lines: Galaxies, Surveys, Astrophysics},
         year = 2005,
        month = dec,
       volume = {130},
       number = {6},
        pages = {2598-2612},
          doi = {10.1086/497431},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508301},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AJ....130.2598G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020MNRAS.498..883G,
       author = {{Grasha}, Kathryn and {Darling}, Jeremy and {Leroy}, Adam K. and
         {Bolatto}, Alberto D.},
        title = "{The evolution of neutral hydrogen over the past 11 Gyr via H I 21 cm absorption}",
      journal = {\mnras},
     keywords = {stars: evolution, galaxies: high-redshift, galaxies: ISM, quasars: absorption lines, cosmology: observations, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = aug,
       volume = {498},
       number = {1},
        pages = {883-898},
          doi = {10.1093/mnras/staa2521},
archivePrefix = {arXiv},
       eprint = {2008.07578},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498..883G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.452.3726H,
       author = {{Hoppmann}, L. and {Staveley-Smith}, L. and {Freudling}, W. and {Zwaan}, M.~A. and {Minchin}, R.~F. and {Calabretta}, M.~R.},
        title = "{A blind H I mass function from the Arecibo Ultra-Deep Survey (AUDS)}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = oct,
       volume = {452},
       number = {4},
        pages = {3726-3741},
          doi = {10.1093/mnras/stv1084},
archivePrefix = {arXiv},
       eprint = {1506.05931},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.452.3726H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2016mks..confE...6J,
       author = {{Jarvis}, M. and {Taylor}, R. and {Agudo}, I. and {Allison}, J.~R. and {Deane}, R.~P. and {Frank}, B. and {Gupta}, N. and {Heywood}, I. and {Maddox}, N. and {McAlpine}, K. and {Santos}, M. and {Scaife}, A.~M.~M. and {Vaccari}, M. and {Zwart}, J.~T.~L. and {Adams}, E. and {Bacon}, D.~J. and {Baker}, A.~J. and {Bassett}, B.~A. and {Best}, P.~N. and {Beswick}, R. and {Blyth}, S. and {Brown}, M.~L. and {Bruggen}, M. and {Cluver}, M. and {Colafrancesco}, S. and {Cotter}, G. and {Cress}, C. and {Dav{\'e}}, R. and {Ferrari}, C. and {Hardcastle}, M.~J. and {Hale}, C.~L. and {Harrison}, I. and {Hatfield}, P.~W. and {Klockner}, H.~R. and {Kolwa}, S. and {Malefahlo}, E. and {Marubini}, T. and {Mauch}, T. and {Moodley}, K. and {Morganti}, R. and {Norris}, R.~P. and {Peters}, J.~A. and {Prandoni}, I. and {Prescott}, M. and {Oliver}, S. and {Oozeer}, N. and {Rottgering}, H.~J.~A. and {Seymour}, N. and {Simpson}, C. and {Smirnov}, O. and {Smith}, D.~J.~B.},
        title = "{The MeerKAT International GHz Tiered Extragalactic Exploration (MIGHTEE) Survey}",
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
    booktitle = {MeerKAT Science: On the Pathway to the SKA},
         year = 2016,
        month = jan,
          eid = {6},
        pages = {6},
archivePrefix = {arXiv},
       eprint = {1709.01901},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016mks..confE...6J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.449.1856J,
       author = {{Jones}, Michael G. and {Papastergis}, Emmanouil and {Haynes}, Martha P. and {Giovanelli}, Riccardo},
        title = "{Spectroscopic confusion: its impact on current and future extragalactic H I surveys}",
      journal = {\mnras},
     keywords = {surveys, galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = may,
       volume = {449},
       number = {2},
        pages = {1856-1868},
          doi = {10.1093/mnras/stv429},
archivePrefix = {arXiv},
       eprint = {1502.07359},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449.1856J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.4393J,
       author = {{Jones}, Michael G. and {Papastergis}, Emmanouil and
         {Haynes}, Martha P. and {Giovanelli}, Riccardo},
        title = "{Environmental dependence of the H I mass function in the ALFALFA 70\% catalogue}",
      journal = {\mnras},
     keywords = {galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Apr",
       volume = {457},
       number = {4},
        pages = {4393-4405},
          doi = {10.1093/mnras/stw263},
archivePrefix = {arXiv},
       eprint = {1510.07050},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.4393J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.477....2J,
       author = {{Jones}, Michael G. and {Haynes}, Martha P. and {Giovanelli}, Riccardo and {Moorman}, Crystal},
        title = "{The ALFALFA H I mass function: a dichotomy in the low-mass slope and a locally suppressed `knee' mass}",
      journal = {\mnras},
     keywords = {surveys, galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jun,
       volume = {477},
       number = {1},
        pages = {2-17},
          doi = {10.1093/mnras/sty521},
archivePrefix = {arXiv},
       eprint = {1802.00053},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477....2J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019SCPMA..6259502J,
       author = {{Jiang}, Peng and {Yue}, YouLing and {Gan}, HengQian and {Yao}, Rui and {Li}, Hui and {Pan}, GaoFeng and {Sun}, JingHai and {Yu}, DongJun and {Liu}, HongFei and {Tang}, NingYu and {Qian}, Lei and {Lu}, JiGuang and {Yan}, Jun and {Peng}, Bo and {Zhang}, ShuXin and {Wang}, QiMing and {Li}, Qi and {Li}, Di},
        title = "{Commissioning progress of the FAST}",
      journal = {Science China Physics, Mechanics, and Astronomy},
     keywords = {radio telescopes and instrumentation, astronomical observations, radio wave receivers, algorithms and implementation, control systems, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = may,
       volume = {62},
       number = {5},
          eid = {959502},
        pages = {959502},
          doi = {10.1007/s11433-018-9376-1},
archivePrefix = {arXiv},
       eprint = {1903.06324},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019SCPMA..6259502J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020RAA....20...64J,
       author = {{Jiang}, Peng and {Tang}, Ning-Yu and {Hou}, Li-Gang and {Liu}, Meng-Ting and {Kr{\v{c}}o}, Marko and {Qian}, Lei and {Sun}, Jing-Hai and {Ching}, Tao-Chung and {Liu}, Bin and {Duan}, Yan and {Yue}, You-Ling and {Gan}, Heng-Qian and {Yao}, Rui and {Li}, Hui and {Pan}, Gao-Feng and {Yu}, Dong-Jun and {Liu}, Hong-Fei and {Li}, Di and {Peng}, Bo and {Yan}, Jun and {FAST Collaboration}},
        title = "{The fundamental performance of FAST with 19-beam receiver at L band}",
      journal = {Research in Astronomy and Astrophysics},
     keywords = {instrumentation: detectors, line: profiles, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = may,
       volume = {20},
       number = {5},
          eid = {064},
        pages = {064},
          doi = {10.1088/1674-4527/20/5/64},
archivePrefix = {arXiv},
       eprint = {2002.01786},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020RAA....20...64J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ARA&A..50..531K,
       author = {{Kennicutt}, Robert C. and {Evans}, Neal J.},
        title = "{Star Formation in the Milky Way and Nearby Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = sep,
       volume = {50},
        pages = {531-608},
          doi = {10.1146/annurev-astro-081811-125610},
archivePrefix = {arXiv},
       eprint = {1204.3552},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ARA&A..50..531K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.453.2315K,
       author = {{Kim}, Han-Seek and {Wyithe}, J.~S.~B. and {Power}, C. and
         {Park}, Jaehong and {Lagos}, C. d. P. and {Baugh}, C.~M.},
        title = "{The H I mass function as a probe of photoionization feedback on low-mass galaxy formation}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, large-scale structure of Universe, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = nov,
       volume = {453},
       number = {3},
        pages = {2315-2325},
          doi = {10.1093/mnras/stv1822},
archivePrefix = {arXiv},
       eprint = {1506.02736},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.2315K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020Ap&SS.365..118K,
       author = {{Koribalski}, B{\"a}rbel S. and {Staveley-Smith}, L. and
         {Westmeier}, T. and {Serra}, P. and {Spekkens}, K. and {Wong}, O.~I. and
         {Lee-Waddell}, K. and {Lagos}, C.~D.~P. and {Obreschkow}, D. and
         {Ryan-Weber}, E.~V. and {Zwaan}, M. and {Kilborn}, V. and
         {Bekiaris}, G. and {Bekki}, K. and {Bigiel}, F. and {Boselli}, A. and
         {Bosma}, A. and {Catinella}, B. and {Chauhan}, G. and {Cluver}, M.~E. and
         {Colless}, M. and {Courtois}, H.~M. and {Crain}, R.~A. and
         {de Blok}, W.~J.~G. and {D{\'e}nes}, H. and {Duffy}, A.~R. and
         {Elagali}, A. and {Fluke}, C.~J. and {For}, B. -Q. and {Heald}, G. and
         {Henning}, P.~A. and {Hess}, K.~M. and {Holwerda}, B.~W. and
         {Howlett}, C. and {Jarrett}, T. and {Jones}, D.~H. and {Jones}, M.~G. and
         {J{\'o}zsa}, G.~I.~G. and {Jurek}, R. and {J{\"u}tte}, E. and
         {Kamphuis}, P. and {Karachentsev}, I. and {Kerp}, J. and {Kleiner}, D. and
         {Kraan-Korteweg}, R.~C. and {L{\'o}pez-S{\'a}nchez}, {\'A}. R. and
         {Madrid}, J. and {Meyer}, M. and {Mould}, J. and {Murugeshan}, C. and
         {Norris}, R.~P. and {Oh}, S. -H. and {Oosterloo}, T.~A. and
         {Popping}, A. and {Putman}, M. and {Reynolds}, T.~N. and {Rhee}, J. and
         {Robotham}, A.~S.~G. and {Ryder}, S. and {Schr{\"o}der}, A.~C. and
         {Shao}, Li and {Stevens}, A.~R.~H. and {Taylor}, E.~N. and
         {van{\^A} der Hulst}, J.~M. and {Verdes-Montenegro}, L. and
         {Wakker}, B.~P. and {Wang}, J. and {Whiting}, M. and {Winkel}, B. and
         {Wolf}, C.},
        title = "{WALLABY - an SKA Pathfinder HI survey}",
      journal = {\apss},
     keywords = {Radio lines: galaxies, ISM, surveys, galaxies: evolution, formation, kinematics \& dynamics, large-scale structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = jul,
       volume = {365},
       number = {7},
          eid = {118},
        pages = {118},
          doi = {10.1007/s10509-020-03831-4},
archivePrefix = {arXiv},
       eprint = {2002.07311},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Ap&SS.365..118K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.376.1357L,
       author = {{Lah}, Philip and {Chengalur}, Jayaram N. and {Briggs}, Frank H. and
         {Colless}, Matthew and {de Propris}, Roberto and {Pracy}, Michael B. and
         {de Blok}, W.~J.~G. and {Fujita}, Shinobu S. and {Ajiki}, Masaru and
         {Shioya}, Yasuhiro and {Nagao}, Tohru and {Murayama}, Takashi and
         {Taniguchi}, Yoshiaki and {Yagi}, Masafumi and {Okamura}, Sadanori},
        title = "{The HI content of star-forming galaxies at z = 0.24}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, radio continuum: galaxies, radio lines: galaxies, Astrophysics},
         year = 2007,
        month = apr,
       volume = {376},
       number = {3},
        pages = {1357-1366},
          doi = {10.1111/j.1365-2966.2007.11540.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701668},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.376.1357L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2019BAAS...51g..57L,
       author = {{Levi}, Michael and {Allen}, Lori E. and {Raichoor}, Anand and {Baltay}, Charles and {BenZvi}, Segev and {Beutler}, Florian and {Bolton}, Adam and {Castander}, Francisco J. and {Chuang}, Chia-Hsun and {Cooper}, Andrew and {Cuby}, Jean-Gabriel and {Dey}, Arjun and {Eisenstein}, Daniel and {Fan}, Xiaohui and {Flaugher}, Brenna and {Frenk}, Carlos and {Gonzalez-Morales}, Alma X. and {Graur}, Or and {Guy}, Julien and {Habib}, Salman and {Honscheid}, Klaus and {Juneau}, Stephanie and {Kneib}, Jean-Paul and {Lahav}, Ofer and {Lang}, Dustin and {Leauthaud}, Alexie and {Lusso}, Betta and {de la Macorra}, Axel and {Manera}, Marc and {Martini}, Paul and {Mao}, Shude and {Newman}, Jeffrey A. and {Palanque-Delabrouille}, Nathalie and {Percival}, Will J. and {Allende Prieto}, Carlos and {Rockosi}, Constance M. and {Ruhlmann-Kleider}, Vanina and {Schlegel}, David and {Seo}, Hee-Jong and {Song}, Yong-Seon and {Tarle}, Greg and {Wechsler}, Risa and {Weinberg}, David and {Yeche}, Christophe and {Zu}, Ying},
        title = "{The Dark Energy Spectroscopic Instrument (DESI)}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Bulletin of the American Astronomical Society},
         year = 2019,
       volume = {51},
        month = sep,
          eid = {57},
        pages = {57},
archivePrefix = {arXiv},
       eprint = {1907.10688},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019BAAS...51g..57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018IMMag..19..112L,
       author = {{Li}, Di and {Wang}, Pei and {Qian}, Lei and {Krco}, Marko and {Jiang}, Peng and {Yue}, Youling and {Jin}, Chenjin and {Zhu}, Yan and {Pan}, Zhichen and {Nan}, Rendong and {Dunning}, Alex},
        title = "{FAST in Space: Considerations for a Multibeam, Multipurpose Survey Using China's 500-m Aperture Spherical Radio Telescope (FAST)}",
      journal = {IEEE Microwave Magazine},
     keywords = {L-band, Imaging, Sensitivity, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = apr,
       volume = {19},
       number = {3},
        pages = {112-119},
          doi = {10.1109/MMM.2018.2802178},
archivePrefix = {arXiv},
       eprint = {1802.03709},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018IMMag..19..112L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...460L...1L,
       author = {{Lilly}, S.~J. and {Le Fevre}, O. and {Hammer}, F. and {Crampton}, David},
        title = "{The Canada-France Redshift Survey: The Luminosity Density and Star Formation History of the Universe to Z approximately 1}",
      journal = {\apjl},
     keywords = {GALAXIES: EVOLUTION, COSMOLOGY: OBSERVATIONS, Astrophysics},
         year = 1996,
        month = mar,
       volume = {460},
        pages = {L1},
          doi = {10.1086/309975},
archivePrefix = {arXiv},
       eprint = {astro-ph/9601050},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...460L...1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...498..106M,
       author = {{Madau}, Piero and {Pozzetti}, Lucia and {Dickinson}, Mark},
        title = "{The Star Formation History of Field Galaxies}",
      journal = {\apj},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: PHOTOMETRY, COSMOLOGY: THEORY, GALAXIES: STELLAR CONTENT, Cosmology: Theory, Galaxies: Evolution, Galaxies: Photometry, Galaxies: Stellar Content, Astrophysics},
         year = 1998,
        month = may,
       volume = {498},
       number = {1},
        pages = {106-116},
          doi = {10.1086/305523},
archivePrefix = {arXiv},
       eprint = {astro-ph/9708220},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...498..106M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...763L..20M,
       author = {{Masui}, K.~W. and {Switzer}, E.~R. and {Banavar}, N. and {Bandura}, K. and
         {Blake}, C. and {Calin}, L. -M. and {Chang}, T. -C. and {Chen}, X. and
         {Li}, Y. -C. and {Liao}, Y. -W. and {Natarajan}, A. and {Pen}, U. -L. and
         {Peterson}, J.~B. and {Shaw}, J.~R. and {Voytek}, T.~C.},
        title = "{Measurement of 21 cm Brightness Fluctuations at z \raisebox{-0.5ex}\textasciitilde 0.8 in Cross-correlation}",
      journal = {\apjl},
     keywords = {galaxies: evolution, large-scale structure of universe, radio lines: galaxies, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2013,
        month = jan,
       volume = {763},
       number = {1},
          eid = {L20},
        pages = {L20},
          doi = {10.1088/2041-8205/763/1/L20},
archivePrefix = {arXiv},
       eprint = {1208.0331},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...763L..20M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.350.1195M,
       author = {{Meyer}, M.~J. and {Zwaan}, M.~A. and {Webster}, R.~L. and
         {Staveley-Smith}, L. and {Ryan-Weber}, E. and {Drinkwater}, M.~J. and
         {Barnes}, D.~G. and {Howlett}, M. and {Kilborn}, V.~A. and
         {Stevens}, J. and {Waugh}, M. and {Pierce}, M.~J. and {Bhathal}, R. and
         {de Blok}, W.~J.~G. and {Disney}, M.~J. and {Ekers}, R.~D. and
         {Freeman}, K.~C. and {Garcia}, D.~A. and {Gibson}, B.~K. and
         {Harnett}, J. and {Henning}, P.~A. and {Jerjen}, H. and
         {Kesteven}, M.~J. and {Knezek}, P.~M. and {Koribalski}, B.~S. and
         {Mader}, S. and {Marquarding}, M. and {Minchin}, R.~F. and
         {O'Brien}, J. and {Oosterloo}, T. and {Price}, R.~M. and
         {Putman}, M.~E. and {Ryder}, S.~D. and {Sadler}, E.~M. and
         {Stewart}, I.~M. and {Stootman}, F. and {Wright}, A.~E.},
        title = "{The HIPASS catalogue - I. Data presentation}",
      journal = {\mnras},
     keywords = {methods: observational, catalogues, surveys, radio lines: galaxies, Astrophysics},
         year = "2004",
        month = "Jun",
       volume = {350},
       number = {4},
        pages = {1195-1209},
          doi = {10.1111/j.1365-2966.2004.07710.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0406384},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.350.1195M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PRA...........M,
       author = {{Meyer}, M. and {Heald}, G. and {Serra}, P.},
        title = "{Wide-field 1–2 GHz Research on Galaxy Evolution}",
      journal = {Proceedings of Panoramic Radio Astronomy},
     keywords = {},
         year = "2009",
          url = {https://pos.sissa.it/cgi-bin/reader/conf.cgi?confid=89}
}

@ARTICLE{2010ApJ...723.1359M,
       author = {{Martin}, Ann M. and {Papastergis}, Emmanouil and {Giovanelli}, Riccardo and {Haynes}, Martha P. and {Springob}, Christopher M. and {Stierwalt}, Sabrina},
        title = "{The Arecibo Legacy Fast ALFA Survey. X. The H I Mass Function and {\ensuremath{\Omega}}\_H I from the 40\% ALFALFA Survey}",
      journal = {\apj},
     keywords = {galaxies: distances and redshifts, galaxies: dwarf, galaxies: luminosity function, mass function, radio lines: galaxies, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = nov,
       volume = {723},
       number = {2},
        pages = {1359-1374},
          doi = {10.1088/0004-637X/723/2/1359},
archivePrefix = {arXiv},
       eprint = {1008.5107},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...723.1359M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.444.3559M,
       author = {{Moorman}, Crystal M. and {Vogeley}, Michael S. and {Hoyle}, Fiona and
         {Pan}, Danny C. and {Haynes}, Martha P. and {Giovanelli}, Riccardo},
        title = "{The H I mass function and velocity width function of void galaxies in the Arecibo Legacy Fast ALFA Survey}",
      journal = {\mnras},
     keywords = {methods: statistical, galaxies: distances and redshifts, galaxies: luminosity function, mass function, cosmology: observations, large-scale structure of Universe, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Nov",
       volume = {444},
       number = {4},
        pages = {3559-3570},
          doi = {10.1093/mnras/stu1674},
archivePrefix = {arXiv},
       eprint = {1408.3392},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444.3559M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011IJMPD..20..989N,
       author = {{Nan}, Rendong and {Li}, Di and {Jin}, Chengjin and {Wang}, Qiming and {Zhu}, Lichun and {Zhu}, Wenbai and {Zhang}, Haiyan and {Yue}, Youling and {Qian}, Lei},
        title = "{The Five-Hundred Aperture Spherical Radio Telescope (fast) Project}",
      journal = {International Journal of Modern Physics D},
     keywords = {Radio telescope, active main reflector, HI 21cm line, pulsar, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {20},
       number = {6},
        pages = {989-1024},
          doi = {10.1142/S0218271811019335},
archivePrefix = {arXiv},
       eprint = {1105.3794},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011IJMPD..20..989N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...698.1467O,
       author = {{Obreschkow}, D. and {Croton}, D. and {De Lucia}, G. and {Khochfar}, S. and {Rawlings}, S.},
        title = "{Simulation of the Cosmic Evolution of Atomic and Molecular Hydrogen in Galaxies}",
      journal = {\apj},
     keywords = {ISM: atoms, ISM: clouds, ISM: molecules, radio lines: galaxies, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2009,
        month = jun,
       volume = {698},
       number = {2},
        pages = {1467-1484},
          doi = {10.1088/0004-637X/698/2/1467},
archivePrefix = {arXiv},
       eprint = {0904.2221},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...698.1467O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022MNRAS.509.3268O,
       author = {{Oman}, Kyle A.},
        title = "{The ALFALFA H I velocity width function}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: luminosity function, mass function, dark matter, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jan,
       volume = {509},
       number = {3},
        pages = {3268-3284},
          doi = {10.1093/mnras/stab3164},
archivePrefix = {arXiv},
       eprint = {2108.08856},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.509.3268O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1965MmRAS..69..183P,
       author = {{Pilkington}, J.~D.~H. and {Scott}, J.~F.},
        title = "{A survey of radio sources between declinations 20{\textdegree} and 40{\textdegree}}",
      journal = {\memras},
         year = 1965,
        month = jan,
       volume = {69},
        pages = {183},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1965MmRAS..69..183P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..197...28P,
       author = {{Pisano}, D.~J. and {Barnes}, David G. and {Staveley-Smith}, Lister and {Gibson}, Brad K. and {Kilborn}, Virginia A. and {Freeman}, Ken C.},
        title = "{An H I Survey of Six Local Group Analogs. II. H I Properties of Group Galaxies}",
      journal = {\apjs},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: groups: general, galaxies: luminosity function, mass function, Local Group, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {197},
       number = {2},
          eid = {28},
        pages = {28},
          doi = {10.1088/0067-0049/197/2/28},
archivePrefix = {arXiv},
       eprint = {1110.3431},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..197...28P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...696.1543P,
       author = {{Prochaska}, J. Xavier and {Wolfe}, Arthur M.},
        title = "{On the (Non)Evolution of H I Gas in Galaxies Over Cosmic Time}",
      journal = {\apj},
     keywords = {galaxies: evolution, intergalactic medium, quasars: absorption lines, Astrophysics},
         year = 2009,
        month = may,
       volume = {696},
       number = {2},
        pages = {1543-1547},
          doi = {10.1088/0004-637X/696/2/1543},
archivePrefix = {arXiv},
       eprint = {0811.2003},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...696.1543P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJS..130....1R,
       author = {{Rao}, Sandhya M. and {Turnshek}, David A.},
        title = "{Discovery of DampedLy{\ensuremath{\alpha}} Systems at Redshifts Less than 1.65 and Results on Their Incidence and Cosmological Mass Density}",
      journal = {\apjs},
     keywords = {Cosmology: Observations, Galaxies: Formation, Galaxies: Quasars: Absorption Lines, Surveys, Astrophysics},
         year = 2000,
        month = sep,
       volume = {130},
       number = {1},
        pages = {1-35},
          doi = {10.1086/317344},
archivePrefix = {arXiv},
       eprint = {astro-ph/9909164},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJS..130....1R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.435.2693R,
       author = {{Rhee}, J. and {Zwaan}, Martin A. and {Briggs}, Frank H. and {Chengalur}, Jayaram N. and {Lah}, Philip and {Oosterloo}, Tom and {van der Hulst}, Thijs},
        title = "{Neutral atomic hydrogen (H I) gas evolution in field galaxies at z {\ensuremath{\sim}} 0.1 and {\ensuremath{\sim}}0.2}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, radio lines: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = nov,
       volume = {435},
       number = {3},
        pages = {2693-2706},
          doi = {10.1093/mnras/stt1481},
archivePrefix = {arXiv},
       eprint = {1308.1462},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.2693R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.473.1879R,
       author = {{Rhee}, Jonghwan and {Lah}, Philip and {Briggs}, Frank H. and {Chengalur}, Jayaram N. and {Colless}, Matthew and {Willner}, Steven P. and {Ashby}, Matthew L.~N. and {Le F{\`e}vre}, Olivier},
        title = "{Neutral hydrogen (H I) gas content of galaxies at z {\ensuremath{\approx}} 0.32}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {473},
       number = {2},
        pages = {1879-1894},
          doi = {10.1093/mnras/stx2461},
archivePrefix = {arXiv},
       eprint = {1709.07596},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.1879R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...567..247R,
       author = {{Rosenberg}, Jessica L. and {Schneider}, Stephen E.},
        title = "{The Arecibo Dual-Beam Survey: The H I Mass Function of Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: ISM, Galaxies: Luminosity Function, Mass Function, Radio Lines: Galaxies, Astrophysics},
         year = 2002,
        month = mar,
       volume = {567},
       number = {1},
        pages = {247-257},
          doi = {10.1086/338377},
archivePrefix = {arXiv},
       eprint = {astro-ph/0111004},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...567..247R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019MNRAS.486.1796S,
       author = {{Said}, Khaled and {Kraan-Korteweg}, Ren{\'e}e C. and
         {Staveley-Smith}, Lister},
        title = "{The H I mass function in the Parkes H I Zone of Avoidance survey}",
      journal = {\mnras},
     keywords = {galaxies: distances and redshifts, large-scale structure of Universe, cosmology: observations, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2019",
        month = "Jun",
       volume = {486},
       number = {2},
        pages = {1796-1804},
          doi = {10.1093/mnras/stz956},
archivePrefix = {arXiv},
       eprint = {1904.01581},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.1796S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.462.1749S,
       author = {{Saintonge}, Amelie and {Catinella}, Barbara and {Cortese}, Luca and
         {Genzel}, Reinhard and {Giovanelli}, Riccardo and {Haynes}, Martha P. and
         {Janowiecki}, Steven and {Kramer}, Carsten and {Lutz}, Katharina A. and
         {Schiminovich}, David and {Tacconi}, Linda J. and {Wuyts}, Stijn and
         {Accurso}, Gioacchino},
        title = "{Molecular and atomic gas along and across the main sequence of star-forming galaxies}",
      journal = {\mnras},
     keywords = {ISM: general, galaxies: evolution, galaxies: ISM, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {462},
       number = {2},
        pages = {1749-1756},
          doi = {10.1093/mnras/stw1715},
archivePrefix = {arXiv},
       eprint = {1607.05289},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.1749S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976ApJ...203..297S,
       author = {{Schechter}, P.},
        title = "{An analytic expression for the luminosity function for galaxies.}",
      journal = {\apj},
         year = "1976",
        month = "Jan",
       volume = {203},
        pages = {297-306},
          doi = {10.1086/154079},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976ApJ...203..297S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1968ApJ...151..393S,
       author = {{Schmidt}, Maarten},
        title = "{Space Distribution and Luminosity Functions of Quasi-Stellar Radio Sources}",
      journal = {\apj},
         year = 1968,
        month = feb,
       volume = {151},
        pages = {393},
          doi = {10.1086/149446},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1968ApJ...151..393S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...621..215S,
       author = {{Springob}, Christopher M. and {Haynes}, Martha P. and
         {Giovanelli}, Riccardo},
        title = "{Morphology, Environment, and the H I Mass Function}",
      journal = {\apj},
     keywords = {Galaxies: Distances and Redshifts, Galaxies: Luminosity Function, Mass Function, Radio Lines: Galaxies, Astrophysics},
         year = "2005",
        month = "Mar",
       volume = {621},
       number = {1},
        pages = {215-226},
          doi = {10.1086/427432},
archivePrefix = {arXiv},
       eprint = {astro-ph/0411349},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...621..215S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996PASA...13..243S,
       author = {{Staveley-Smith}, L. and {Wilson}, W.~E. and {Bird}, T.~S. and {Disney}, M.~J. and {Ekers}, R.~D. and {Freeman}, K.~C. and {Haynes}, R.~F. and {Sinclair}, M.~W. and {Vaile}, R.~A. and {Webster}, R.~L. and {Wright}, A.~E.},
        title = "{The Parkes 21 CM multibeam receiver}",
      journal = {\pasa},
     keywords = {INSTRUMENTATION, RECEIVERS},
         year = 1996,
        month = nov,
       volume = {13},
       number = {3},
        pages = {243-248},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996PASA...13..243S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016AJ....151...52S,
       author = {{Staveley-Smith}, L. and {Kraan-Korteweg}, R.~C. and
         {Schr{\"o}der}, A.~C. and {Henning}, P.~A. and {Koribalski}, B.~S. and
         {Stewart}, I.~M. and {Heald}, G.},
        title = "{The Parkes H I Zone of Avoidance Survey}",
      journal = {\aj},
     keywords = {galaxies: distances and redshifts, galaxies: fundamental parameters, large-scale structure of universe, surveys, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2016",
        month = "Mar",
       volume = {151},
       number = {3},
          eid = {52},
        pages = {52},
          doi = {10.3847/0004-6256/151/3/52},
archivePrefix = {arXiv},
       eprint = {1602.02922},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016AJ....151...52S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.438.1176W,
       author = {{Westmeier}, T. and {Jurek}, R. and {Obreschkow}, D. and
         {Koribalski}, B.~S. and {Staveley-Smith}, L.},
        title = "{The busy function: a new analytic function for describing the integrated 21-cm spectral profile of galaxies}",
      journal = {\mnras},
     keywords = {line: profiles, methods: data analysis, radio lines: galaxies, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Feb",
       volume = {438},
       number = {2},
        pages = {1176-1190},
          doi = {10.1093/mnras/stt2266},
archivePrefix = {arXiv},
       eprint = {1311.5308},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.438.1176W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.472.4832W,
       author = {{Westmeier}, T. and {Obreschkow}, D. and {Calabretta}, M. and {Jurek}, R. and {Koribalski}, B.~S. and {Meyer}, M. and {Musaeva}, A. and {Popping}, A. and {Staveley-Smith}, L. and {Wong}, O.~I. and {Wright}, A.},
        title = "{A deep Parkes H I survey of the Sculptor group and filament: H I mass function and environment}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: groups: individual: Sculptor group, galaxies: ISM, galaxies: luminosity function, mass function, radio lines: galaxies, mass function - radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = dec,
       volume = {472},
       number = {4},
        pages = {4832-4850},
          doi = {10.1093/mnras/stx2289},
archivePrefix = {arXiv},
       eprint = {1709.00780},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472.4832W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2013tra..book.....W,
       author = {{Wilson}, Thomas L. and {Rohlfs}, Kristen and {H{\"u}ttemeister}, Susanne},
        title = "{Tools of Radio Astronomy}",
         year = 2013,
          doi = {10.1007/978-3-642-39950-3},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013tra..book.....W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.501.4550X,
       author = {{Xi}, Hongwei and {Staveley-Smith}, Lister and {For}, Bi-Qing and {Freudling}, Wolfram and {Zwaan}, Martin and {Hoppmann}, Laura and {Liang}, Fu-Heng and {Peng}, Bo},
        title = "{The Arecibo Ultra-Deep Survey}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = mar,
       volume = {501},
       number = {3},
        pages = {4550-4564},
          doi = {10.1093/mnras/staa3931},
archivePrefix = {arXiv},
       eprint = {2012.09516},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.4550X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019SCPMA..6259506Z,
       author = {{Zhang}, Kai and {Wu}, JingWen and {Li}, Di and {Kr{\v{c}}o}, Marko and {Staveley-Smith}, Lister and {Tang}, NingYu and {Qian}, Lei and {Liu}, MengTing and {Jin}, ChengJin and {Yue}, YouLing and {Zhu}, Yan and {Liu}, HongFei and {Yu}, DongJun and {Sun}, JingHai and {Pan}, GaoFeng and {Li}, Hui and {Gan}, HengQian and {Yao}, Rui},
        title = "{Status and perspectives of the CRAFTS extra-galactic HI survey}",
      journal = {Science China Physics, Mechanics, and Astronomy},
     keywords = {HI regions and 21-cm lines, radio telescopes and instrumentation, statistical and correlative studies of properties, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {62},
       number = {5},
          eid = {959506},
        pages = {959506},
          doi = {10.1007/s11433-019-9383-y},
archivePrefix = {arXiv},
       eprint = {1903.06402},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019SCPMA..6259506Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.500.1741Z,
       author = {{Zhang}, Kai and {Wu}, Jingwen and {Li}, Di and {Tsai}, Chao-Wei and {Staveley-Smith}, Lister and {Wang}, Jing and {Fu}, Jian and {McIntyre}, Travis and {Yuan}, Mao},
        title = "{Predictions for the FAST telescope's CRAFTS extragalactic H I survey}",
      journal = {\mnras},
     keywords = {surveys, galaxies: luminosity function, mass function, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jan,
       volume = {500},
       number = {2},
        pages = {1741-1754},
          doi = {10.1093/mnras/staa3275},
archivePrefix = {arXiv},
       eprint = {2012.01683},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.1741Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003AJ....125.2842Z,
       author = {{Zwaan}, M.~A. and {Staveley-Smith}, L. and {Koribalski}, B.~S. and
         {Henning}, P.~A. and {Kilborn}, V.~A. and {Ryder}, S.~D. and
         {Barnes}, D.~G. and {Bhathal}, R. and {Boyce}, P.~J. and
         {de Blok}, W.~J.~G. and {Disney}, M.~J. and {Drinkwater}, M.~J. and
         {Ekers}, R.~D. and {Freeman}, K.~C. and {Gibson}, B.~K. and
         {Green}, A.~J. and {Haynes}, R.~F. and {Jerjen}, H. and {Juraszek}, S. and
         {Kesteven}, M.~J. and {Knezek}, P.~M. and {Kraan-Korteweg}, R.~C. and
         {Mader}, S. and {Marquarding}, M. and {Meyer}, M. and {Minchin}, R.~F. and
         {Mould}, J.~R. and {O'Brien}, J. and {Oosterloo}, T. and
         {Price}, R.~M. and {Putman}, M.~E. and {Ryan-Weber}, E. and
         {Sadler}, E.~M. and {Schr{\"o}der}, A. and {Stewart}, I.~M. and
         {Stootman}, F. and {Warren}, B. and {Waugh}, M. and {Webster}, R.~L. and
         {Wright}, A.~E.},
        title = "{The 1000 Brightest HIPASS Galaxies: The H I Mass Function and {\ensuremath{\Omega}}$_{HI}$}",
      journal = {\aj},
     keywords = {Galaxies: ISM, Galaxies: Luminosity Function, Mass Function, ISM: General, Radio Emission Lines, Surveys, Astrophysics},
         year = "2003",
        month = "Jun",
       volume = {125},
       number = {6},
        pages = {2842-2858},
          doi = {10.1086/374944},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302440},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003AJ....125.2842Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.359L..30Z,
       author = {{Zwaan}, M.~A. and {Meyer}, M.~J. and {Staveley-Smith}, L. and
         {Webster}, R.~L.},
        title = "{The HIPASS catalogue: {\ensuremath{\Omega}}$_{HI}$ and environmental effects on the HI mass function of galaxies}",
      journal = {\mnras},
     keywords = {methods: observational, methods: statistical, surveys, galaxies: luminosity function, mass function, galaxies: statistics, radio lines: galaxies, Astrophysics},
         year = "2005",
        month = "May",
       volume = {359},
       number = {1},
        pages = {L30-L34},
          doi = {10.1111/j.1745-3933.2005.00029.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502257},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.359L..30Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001Sci...293.1800Z,
       author = {{Zwaan}, M.~A. and {van Dokkum}, P.~G. and {Verheijen}, M.~A.~W.},
        title = "{Hydrogen 21-Centimeter Emission from a Galaxy at Cosmological Distance}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics},
         year = 2001,
        month = sep,
       volume = {293},
       number = {5536},
        pages = {1800-1803},
          doi = {10.1126/science.1063034},
archivePrefix = {arXiv},
       eprint = {astro-ph/0109108},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001Sci...293.1800Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
